Nowcasting with Mixed Frequency Data Using Gaussian Processes

We develop Bayesian machine learning methods for mixed data sampling (MIDAS) regressions. This involves handling frequency mismatches and specifying functional relationships between many predictors and the dependent variable. We use Gaussian processes (GPs) and compress the input space with structured and unstructured MIDAS variants. This yields several versions of GP-MIDAS with distinct properties and implications, which we evaluate in short-horizon now- and forecasting exercises with both simulated data and data on quarterly US output growth and inflation in the GDP deflator. It turns out that our proposed framework leverages macroeconomic Big Data in a computationally efficient way and offers gains in predictive accuracy compared to other machine learning approaches along several dimensions.

==> tabs/CRPS_poster.tex <==



==> tabs/GDPC1_q_CRPStab.tex <==
%latex.default(CRPS.tab, file = paste0(save.dir, sl.endo, "_CRPStab.tex"),     title = "", ctable = FALSE, n.rgroup = n.rgroup, rgroup = rgroup,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     caption = paste0("CRPS: ", sl.endo), label = "tab:eval",     size = "tiny", booktabs = TRUE, rowname = "", numeric.dollar = FALSE,     caption.loc = "bottom", landscape = FALSE, dcolumn = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries now}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries one-step-ahead}\tabularnewline
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Midas}&\multicolumn{1}{c}{Variance}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}\tabularnewline
\midrule
{\bfseries }&&&&&&&&&&&\tabularnewline
~~&bart&almon&sv&&1.008&1.064&1.108&&1.026&1.008&1.047\tabularnewline
~~&&&homosc.&&1.026&1.082&1.097&&1.042&1.006&1.047\tabularnewline
~~&&beta&sv&&1.027&1.039&1.199&&1.078&0.961&1.162\tabularnewline
~~&&&homosc.&&1.065&1.064&1.186&&1.073&1.058&1.156\tabularnewline
~~&&n&sv&&1.030&1.051&1.186&&1.082&1.084&1.139\tabularnewline
~~&&&homosc.&&1.031&1.058&1.178&&1.094&1.097&1.150\tabularnewline
~~&&u&sv&&1.127&1.150&1.140&&1.005&1.011&1.057\tabularnewline
~~&&&homosc.&&1.130&1.127&1.144&&1.019&0.998&1.049\tabularnewline
~~&GP (matern)&almon&sv&&0.988&0.994&1.158&&1.003&0.943&0.999\tabularnewline
~~&&&homosc.&&0.957&0.927&1.109&&0.977&0.919&0.990\tabularnewline
~~&&beta&sv&&0.944&0.910&1.108&&1.051&1.047&1.124\tabularnewline
~~&&&homosc.&&0.929&\textbf{0.886}&1.091&&1.012&1.084&1.145\tabularnewline
~~&&n&sv&&1.038&1.002&1.152&&1.068&1.060&1.117\tabularnewline
~~&&&homosc.&&1.025&0.969&1.117&&1.024&1.080&1.111\tabularnewline
~~&&u&sv&&1.317&1.404&1.164&&1.175&1.250&1.100\tabularnewline
~~&&&homosc.&&1.322&1.433&1.124&&1.169&1.217&1.062\tabularnewline
~~&GP (sqexp)&almon&sv&&0.998&0.998&1.159&&1.020&0.948&1.009\tabularnewline
~~&&&homosc.&&0.967&0.946&1.126&&1.007&0.937&0.993\tabularnewline
~~&&beta&sv&&0.946&0.911&1.126&&1.052&1.071&1.153\tabularnewline
~~&&&homosc.&&0.931&0.889&1.114&&1.026&1.071&1.172\tabularnewline
~~&&n&sv&&1.045&1.003&1.161&&1.083&1.064&1.132\tabularnewline
~~&&&homosc.&&1.030&0.983&1.147&&1.031&1.076&1.137\tabularnewline
~~&&u&sv&&1.330&1.446&1.160&&1.178&1.247&1.099\tabularnewline
~~&&&homosc.&&1.327&1.461&1.128&&1.182&1.241&1.055\tabularnewline
~~&lin&almon&sv&&0.952&0.937&0.984&&0.922&\textbf{0.901}&0.917\tabularnewline
~~&&&homosc.&&0.990&0.974&1.020&&0.945&0.931&0.940\tabularnewline
~~&&beta&sv&&0.955&0.926&1.057&&0.978&0.980&1.074\tabularnewline
~~&&&homosc.&&0.988&0.963&1.090&&1.032&1.038&1.140\tabularnewline
~~&&n&sv&&0.996&0.985&1.076&&1.008&0.995&1.041\tabularnewline
~~&&&homosc.&&1.027&1.010&1.116&&1.031&1.029&1.098\tabularnewline
~~&&u&sv&&1.018&1.072&1.074&&0.995&1.008&0.956\tabularnewline
~~&&&homosc.&&\shadecell 0.931&1.056&1.085&&\shadecell 1.125&1.033&0.969\tabularnewline
\bottomrule
\end{tabular}}
\caption{real GDP growth}
\end{center}}
\end{table}


==> tabs/GDPC1_q_LPLtab.tex <==
%latex.default(LPL.tab, file = paste0(save.dir, sl.endo, "_LPLtab.tex"),     title = "", ctable = FALSE, n.rgroup = n.rgroup, rgroup = rgroup,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     caption = paste0("LPL: ", sl.endo), label = "tab:eval", size = "tiny",     booktabs = TRUE, rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE, dcolumn = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries now}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries one-step-ahead}\tabularnewline
\cline{2-4} \cline{6-8} \cline{10-12}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Midas}&\multicolumn{1}{c}{Variance}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}\tabularnewline
\midrule
{\bfseries }&&&&&&&&&&&\tabularnewline
~~&bart&almon&sv&&  --4.991&  --7.704&  --9.504&&  --3.298&  --2.610&  --5.510\tabularnewline
~~&bart&almon&homosc.&&  --5.918&  --8.929&  --9.564&&  --5.322&  --3.997&  --5.392\tabularnewline
~~&bart&beta&sv&&  --5.245&  --4.421& --13.784&&  28.766&\textbf{66.158}&  --3.923\tabularnewline
~~&bart&beta&homosc.&&  --7.271&  --8.098& --13.183&&  --7.253&  --8.366& --13.762\tabularnewline
~~&bart&n&sv&&  --4.455&  --6.387& --12.953&&  --7.037&  --8.275& --10.528\tabularnewline
~~&bart&n&homosc.&&  --4.861&  --6.443& --12.507&&  --9.391& --10.732& --13.110\tabularnewline
~~&bart&u&sv&&  --7.692&  --9.776& --10.517&&  --2.022&  --3.731&  --7.099\tabularnewline
~~&bart&u&homosc.&&  --7.597&  --8.611&  --9.870&&  --2.554&  --3.006&  --5.308\tabularnewline
~~&GP (matern)&almon&sv&&--125.043& --59.442&--333.474&& --57.184& --23.739&--206.946\tabularnewline
~~&GP (matern)&almon&homosc.&& --57.560&  --1.283&--161.617&&  --4.238&   7.921& --72.376\tabularnewline
~~&GP (matern)&beta&sv&& --74.705& --18.919&--148.629&& --75.626& --51.775&--128.308\tabularnewline
~~&GP (matern)&beta&homosc.&& --48.172&  --1.649&--107.710&&   0.231&  --1.622& --26.909\tabularnewline
~~&GP (matern)&n&sv&&--120.788& --43.344&--159.576&& --90.734& --54.185&--126.798\tabularnewline
~~&GP (matern)&n&homosc.&& --67.324&  --2.873& --77.305&&  --1.052&  --2.039& --25.788\tabularnewline
~~&GP (matern)&u&sv&& --98.335& --54.590& --73.587&& --73.392& --38.263& --95.168\tabularnewline
~~&GP (matern)&u&homosc.&& --59.207& --49.085& --42.099&&  --9.993& --18.366& --24.880\tabularnewline
~~&GP (sqexp)&almon&sv&&--148.600& --72.506&--390.212&& --94.267& --38.461&--289.012\tabularnewline
~~&GP (sqexp)&almon&homosc.&& --88.512& --28.954&--260.217&& --41.843& --11.782&--224.500\tabularnewline
~~&GP (sqexp)&beta&sv&& --93.085& --26.947&--209.512&&--105.118& --73.140&--191.540\tabularnewline
~~&GP (sqexp)&beta&homosc.&& --68.796& --10.084&--166.630&& --12.368&  --9.713& --72.104\tabularnewline
~~&GP (sqexp)&n&sv&&--139.721& --54.374&--221.720&&--125.015& --71.994&--176.627\tabularnewline
~~&GP (sqexp)&n&homosc.&& --94.530& --26.118&--145.606&& --11.321&  --2.296& --59.501\tabularnewline
~~&GP (sqexp)&u&sv&&--111.315& --68.067& --82.722&& --93.115& --53.490&--109.848\tabularnewline
~~&GP (sqexp)&u&homosc.&& --82.552& --63.072& --55.955&& --24.481& --26.262& --39.495\tabularnewline
~~&lin&almon&sv&&   2.084&   4.678&  --0.436&&   5.133&   6.764&   5.413\tabularnewline
~~&lin&almon&homosc.&&  --1.974&  --1.506&  --5.984&&   1.629&   2.571&   1.194\tabularnewline
~~&lin&beta&sv&&   1.956&   2.979&  --6.557&&   1.096&   2.152&  --5.306\tabularnewline
~~&lin&beta&homosc.&&  --1.571&  --0.736& --10.307&&  --6.155&  --7.128& --13.701\tabularnewline
~~&lin&n&sv&&  --0.607&  --0.390&  --6.546&&   0.232&  --0.022&  --3.361\tabularnewline
~~&lin&n&homosc.&&  --4.098&  --3.693& --11.850&&  --6.117&  --6.343& --11.412\tabularnewline
~~&lin&u&sv&&  --0.637&   2.689&  --4.282&&  --1.259&   3.424&   2.404\tabularnewline
~~&lin&u&homosc.&&--155.903&\textbf{8.870}&  --5.655&&--170.479&   2.228&   0.138\tabularnewline
\bottomrule
\end{tabular}}
\caption{real GDP growth}
\end{center}}
\end{table}


==> tabs/GDPC1_q_MSEtab.tex <==
%latex.default(MSE.tab, file = paste0(save.dir, sl.endo, "_MSEtab.tex"),     title = "", ctable = FALSE, n.rgroup = n.rgroup, rgroup = rgroup,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     caption = paste0("RMSE: ", sl.endo), label = "tab:eval",     size = "tiny", booktabs = TRUE, rowname = "", numeric.dollar = FALSE,     caption.loc = "bottom", landscape = FALSE, dcolumn = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries now}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries one-step-ahead}\tabularnewline
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Midas}&\multicolumn{1}{c}{Variance}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}\tabularnewline
\midrule
{\bfseries }&&&&&&&&&&&\tabularnewline
~~&bart&almon&sv&&1.013&1.072&1.139&&1.053&1.015&1.081\tabularnewline
~~&&&homosc.&&1.013&1.080&1.110&&1.046&0.999&1.058\tabularnewline
~~&&beta&sv&&1.029&1.043&1.253&&1.130&0.961&1.234\tabularnewline
~~&&&homosc.&&1.064&1.063&1.238&&1.084&1.096&1.198\tabularnewline
~~&&n&sv&&1.059&1.098&1.248&&1.100&1.133&1.202\tabularnewline
~~&&&homosc.&&1.043&1.090&1.240&&1.097&1.124&1.189\tabularnewline
~~&&u&sv&&1.167&1.205&1.217&&1.021&1.053&1.123\tabularnewline
~~&&&homosc.&&1.178&1.193&1.224&&1.044&1.037&1.099\tabularnewline
~~&GP (matern)&almon&sv&&0.957&0.994&1.045&&0.963&0.944&0.945\tabularnewline
~~&&&homosc.&&0.956&0.978&1.043&&0.995&0.956&0.970\tabularnewline
~~&&beta&sv&&0.907&0.905&1.057&&1.017&1.065&1.113\tabularnewline
~~&&&homosc.&&0.906&0.900&1.057&&1.052&1.162&1.169\tabularnewline
~~&&n&sv&&0.997&1.001&1.082&&1.014&1.056&1.088\tabularnewline
~~&&&homosc.&&1.004&1.001&1.080&&1.058&1.149&1.130\tabularnewline
~~&&u&sv&&1.238&1.446&1.148&&1.134&1.292&1.120\tabularnewline
~~&&&homosc.&&1.264&1.479&1.130&&1.208&1.288&1.088\tabularnewline
~~&GP (sqexp)&almon&sv&&0.960&0.990&1.036&&0.959&0.937&0.943\tabularnewline
~~&&&homosc.&&0.956&0.975&1.030&&0.992&0.947&0.924\tabularnewline
~~&&beta&sv&&0.901&0.902&1.051&&1.008&1.073&1.121\tabularnewline
~~&&&homosc.&&0.900&\textbf{0.897}&1.051&&1.054&1.133&1.164\tabularnewline
~~&&n&sv&&0.998&0.996&1.073&&1.017&1.045&1.089\tabularnewline
~~&&&homosc.&&1.002&0.994&1.077&&1.047&1.145&1.131\tabularnewline
~~&&u&sv&&1.236&1.473&1.137&&1.122&1.283&1.115\tabularnewline
~~&&&homosc.&&1.250&1.488&1.124&&1.191&1.291&1.071\tabularnewline
~~&lin&almon&sv&&0.984&0.962&1.005&&0.930&\textbf{0.916}&0.933\tabularnewline
~~&&&homosc.&&0.995&0.966&1.009&&0.930&0.916&0.927\tabularnewline
~~&&beta&sv&&0.978&0.943&1.074&&1.017&1.023&1.139\tabularnewline
~~&&&homosc.&&0.996&0.956&1.084&&1.031&1.041&1.178\tabularnewline
~~&&n&sv&&1.023&1.004&1.095&&1.046&1.031&1.102\tabularnewline
~~&&&homosc.&&1.027&1.010&1.107&&1.025&1.026&1.119\tabularnewline
~~&&u&sv&&1.019&1.103&1.094&&1.016&1.042&0.977\tabularnewline
~~&&&homosc.&&\shadecell 1.623&1.085&1.102&&\shadecell 1.965&1.056&0.969\tabularnewline
\bottomrule
\end{tabular}}
\caption{real GDP growth}
\end{center}}
\end{table}


==> tabs/GDPCTPI_q_CRPStab.tex <==
%latex.default(CRPS.tab, file = paste0(save.dir, sl.endo, "_CRPStab.tex"),     title = "", ctable = FALSE, n.rgroup = n.rgroup, rgroup = rgroup,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     caption = paste0("CRPS: ", sl.endo), label = "tab:eval",     size = "tiny", booktabs = TRUE, rowname = "", numeric.dollar = FALSE,     caption.loc = "bottom", landscape = FALSE, dcolumn = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries now}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries one-step-ahead}\tabularnewline
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Midas}&\multicolumn{1}{c}{Variance}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}\tabularnewline
\midrule
{\bfseries }&&&&&&&&&&&\tabularnewline
~~&bart&almon&sv&&1.043&0.980&0.993&&0.867&0.848&0.848\tabularnewline
~~&&&homosc.&&1.116&1.031&1.002&&0.934&0.888&0.866\tabularnewline
~~&&beta&homosc.&&1.073&0.896&1.010&&1.049&0.917&0.956\tabularnewline
~~&&n&sv&&1.131&1.035&1.010&&0.929&0.906&0.911\tabularnewline
~~&&&homosc.&&1.201&1.044&1.055&&1.018&0.952&0.974\tabularnewline
~~&&u&sv&&1.108&0.991&1.035&&0.945&0.849&0.967\tabularnewline
~~&&&homosc.&&1.079&1.018&1.027&&0.975&0.902&0.971\tabularnewline
~~&GP (matern)&almon&sv&&1.027&0.943&1.059&&0.844&0.807&0.867\tabularnewline
~~&&&homosc.&&1.020&0.916&1.031&&0.861&0.830&0.915\tabularnewline
~~&&beta&sv&&0.964&0.879&0.998&&0.895&0.879&0.946\tabularnewline
~~&&&homosc.&&0.914&0.810&0.931&&0.927&0.893&0.974\tabularnewline
~~&&n&sv&&1.041&0.951&1.056&&0.851&0.865&0.888\tabularnewline
~~&&&homosc.&&1.027&0.930&1.008&&0.862&0.891&0.931\tabularnewline
~~&&u&sv&&1.095&1.142&0.981&&1.030&0.972&0.924\tabularnewline
~~&&&homosc.&&1.230&1.212&0.927&&1.206&1.147&0.888\tabularnewline
~~&GP (sqexp)&almon&sv&&1.032&0.946&1.067&&0.854&0.821&0.890\tabularnewline
~~&&&homosc.&&1.025&0.923&1.045&&0.868&0.853&0.812\tabularnewline
~~&&beta&sv&&0.957&0.882&1.000&&0.909&0.883&0.976\tabularnewline
~~&&&homosc.&&0.933&\textbf{0.785}&0.960&&0.913&0.919&0.988\tabularnewline
~~&&n&sv&&1.043&0.958&1.066&&0.876&0.876&0.925\tabularnewline
~~&&&homosc.&&1.036&0.939&1.024&&0.893&0.914&0.891\tabularnewline
~~&&u&sv&&1.087&1.140&0.982&&1.029&0.975&0.925\tabularnewline
~~&&&homosc.&&1.224&1.214&0.932&&1.208&1.160&0.897\tabularnewline
~~&lin&almon&sv&&0.952&0.896&0.964&&0.839&\textbf{0.779}&0.852\tabularnewline
~~&&&homosc.&&1.038&0.933&0.977&&0.946&0.850&0.868\tabularnewline
~~&&beta&sv&&0.923&0.851&0.925&&0.903&0.835&0.919\tabularnewline
~~&&&homosc.&&1.004&0.903&0.982&&1.026&0.947&0.999\tabularnewline
~~&&n&sv&&0.946&0.873&0.946&&0.853&0.808&0.877\tabularnewline
~~&&&homosc.&&1.025&0.917&0.961&&0.932&0.902&0.923\tabularnewline
~~&&u&sv&&0.934&0.917&1.825&&0.875&0.859&1.580\tabularnewline
~~&&&homosc.&& \shadecell 0.511&0.928& 2.141&& \shadecell 0.579&0.962&1.798\tabularnewline
\bottomrule
\end{tabular}}
\caption{Inflation (GDPCTPI)}
\end{center}}
\end{table}


==> tabs/GDPCTPI_q_LPLtab.tex <==
%latex.default(LPL.tab, file = paste0(save.dir, sl.endo, "_LPLtab.tex"),     title = "", ctable = FALSE, n.rgroup = n.rgroup, rgroup = rgroup,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     caption = paste0("LPL: ", sl.endo), label = "tab:eval", size = "tiny",     booktabs = TRUE, rowname = "", numeric.dollar = FALSE, caption.loc = "bottom",     landscape = FALSE, dcolumn = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries now}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries one-step-ahead}\tabularnewline
\cline{2-4} \cline{6-8} \cline{10-12}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Midas}&\multicolumn{1}{c}{Variance}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}\tabularnewline
\midrule
{\bfseries }&&&&&&&&&&&\tabularnewline
~~&bart&almon&sv&&  --2.767&   3.095&   1.213&&  12.400&  12.194&  11.861\tabularnewline
~~&bart&almon&homosc.&&  --5.674&  --0.327&   0.375&&   6.187&   9.067&   9.520\tabularnewline
~~&bart&beta&homosc.&&  --0.741&\textbf{82.091}&   0.234&&   0.116&\textbf{96.046}&   4.881\tabularnewline
~~&bart&n&sv&&  --8.331&  --0.113&  --0.698&&  10.099&   9.784&   6.549\tabularnewline
~~&bart&n&homosc.&& --10.541&   0.887&  --3.553&&   2.075&   7.204&   2.262\tabularnewline
~~&bart&u&sv&&  --4.206&   1.147&   0.559&&   0.380&  12.185&   3.879\tabularnewline
~~&bart&u&homosc.&&  --1.583&   1.267&   1.253&&   4.056&   8.977&   4.343\tabularnewline
~~&GP (matern)&almon&sv&&--252.091& --73.937&--374.754&& --47.030& --20.261&--209.483\tabularnewline
~~&GP (matern)&almon&homosc.&& --90.080& --19.973&--215.780&&   5.028&  13.793& --19.127\tabularnewline
~~&GP (matern)&beta&sv&&--158.405& --45.822&--344.595&& --83.072& --46.713&--265.922\tabularnewline
~~&GP (matern)&beta&homosc.&& --12.673&   4.041& --65.279&&  --1.808&   3.143& --23.512\tabularnewline
~~&GP (matern)&n&sv&&--284.066& --75.665&--496.135&& --46.108& --35.857&--194.233\tabularnewline
~~&GP (matern)&n&homosc.&&--102.898& --21.148&--206.180&&   2.216&   3.801&  --7.538\tabularnewline
~~&GP (matern)&u&sv&& --73.478& --20.999&--188.825&& --48.287&  --8.913&--175.259\tabularnewline
~~&GP (matern)&u&homosc.&& --44.029& --18.331& --32.901&& --22.513& --11.505& --17.106\tabularnewline
~~&GP (sqexp)&almon&sv&&--275.282& --81.334&--433.886&& --96.434& --38.096&--306.612\tabularnewline
~~&GP (sqexp)&almon&homosc.&&--129.572& --33.979&--257.383&& --12.601&   3.816&--104.934\tabularnewline
~~&GP (sqexp)&beta&sv&&--170.190& --51.062&--393.308&&--120.690& --63.936&--407.447\tabularnewline
~~&GP (sqexp)&beta&homosc.&& --59.344&   1.191&--163.685&& --30.724&  --6.714&--118.990\tabularnewline
~~&GP (sqexp)&n&sv&&--317.571& --86.777&--578.711&&--106.815& --57.486&--365.243\tabularnewline
~~&GP (sqexp)&n&homosc.&&--160.864& --37.785&--339.168&& --23.167&  --3.849& --98.568\tabularnewline
~~&GP (sqexp)&u&sv&& --71.542& --21.791&--211.429&& --56.590& --19.906&--198.407\tabularnewline
~~&GP (sqexp)&u&homosc.&& --46.142& --19.419& --67.061&& --25.408& --14.772& --44.390\tabularnewline
~~&lin&almon&sv&&   3.037&   8.859&   4.043&&  11.608&  18.967&  10.954\tabularnewline
~~&lin&almon&homosc.&&  --2.772&   4.924&   1.751&&   3.256&  11.668&   8.666\tabularnewline
~~&lin&beta&sv&&   4.510&  13.015&   7.122&&   5.473&  12.276&   7.537\tabularnewline
~~&lin&beta&homosc.&&   0.383&   7.820&   1.347&&  --2.126&   3.722&  --0.357\tabularnewline
~~&lin&n&sv&&   2.774&   9.563&   4.748&&  10.138&  14.751&  10.734\tabularnewline
~~&lin&n&homosc.&&  --1.576&   6.919&   2.936&&   4.187&   6.730&   5.131\tabularnewline
~~&lin&u&sv&&   5.097&  11.562& --43.998&&   9.019&  14.049& --32.013\tabularnewline
~~&lin&u&homosc.&&--107.216&   9.261& --56.463&&--116.513&   5.169& --44.117\tabularnewline
\bottomrule
\end{tabular}}
\caption{real GDP deflator}
\end{center}}
\end{table}


==> tabs/GDPCTPI_q_MSEtab.tex <==
%latex.default(MSE.tab, file = paste0(save.dir, sl.endo, "_MSEtab.tex"),     title = "", ctable = FALSE, n.rgroup = n.rgroup, rgroup = rgroup,     n.cgroup = n.cgroup, cgroup = cgroup, colheads = colheads,     caption = paste0("RMSE: ", sl.endo), label = "tab:eval",     size = "tiny", booktabs = TRUE, rowname = "", numeric.dollar = FALSE,     caption.loc = "bottom", landscape = FALSE, dcolumn = FALSE)%
\begin{table}[!tbp]
{\tiny
\begin{center}
\scalebox{0.7}{
\begin{tabular}{llllclllclll}
\toprule
\multicolumn{1}{l}{\bfseries }&\multicolumn{3}{c}{\bfseries Specification}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries now}&\multicolumn{1}{c}{\bfseries }&\multicolumn{3}{c}{\bfseries one-step-ahead}\tabularnewline
\cmidrule{2-4} \cmidrule{6-8} \cmidrule{10-12}
\multicolumn{1}{l}{}&\multicolumn{1}{c}{Model}&\multicolumn{1}{c}{Midas}&\multicolumn{1}{c}{Variance}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}&\multicolumn{1}{c}{}&\multicolumn{1}{c}{S}&\multicolumn{1}{c}{M}&\multicolumn{1}{c}{PCA}\tabularnewline
\midrule
{\bfseries }&&&&&&&&&&&\tabularnewline
~~&bart&almon&sv&&1.068&1.005&1.000&&0.872&0.853&0.829\tabularnewline
~~&&&homosc.&&1.154&1.070&0.996&&0.942&0.890&0.838\tabularnewline
~~&&beta&homosc.&&1.105&0.875&0.994&&1.076&0.964&0.945\tabularnewline
~~&&n&sv&&1.155&1.057&0.998&&0.924&0.892&0.883\tabularnewline
~~&&&homosc.&&1.240&1.075&1.040&&1.027&0.941&0.963\tabularnewline
~~&&u&sv&&1.094&0.994&1.053&&0.940&0.812&0.960\tabularnewline
~~&&&homosc.&&1.093&1.020&1.040&&0.981&0.875&0.970\tabularnewline
~~&GP (matern)&almon&sv&&0.944&0.887&0.953&&0.801&0.774&0.782\tabularnewline
~~&&&homosc.&&0.972&0.893&0.950&&0.843&0.815&0.884\tabularnewline
~~&&beta&sv&&0.905&0.830&0.890&&0.832&0.814&0.827\tabularnewline
~~&&&homosc.&&0.917&0.804&0.892&&0.909&0.852&0.933\tabularnewline
~~&&n&sv&&0.947&0.890&0.914&&0.805&0.808&0.788\tabularnewline
~~&&&homosc.&&0.962&0.903&0.908&&0.841&0.863&0.892\tabularnewline
~~&&u&sv&&1.074&1.158&0.875&&1.004&0.978&0.825\tabularnewline
~~&&&homosc.&&1.221&1.238&0.884&&1.231&1.144&0.880\tabularnewline
~~&GP (sqexp)&almon&sv&&0.942&0.883&0.949&&0.798&0.780&0.787\tabularnewline
~~&&&homosc.&&0.963&0.881&0.951&&0.850&0.837&0.773\tabularnewline
~~&&beta&sv&&0.897&0.828&0.890&&0.837&0.812&0.838\tabularnewline
~~&&&homosc.&&0.900&\textbf{0.762}&0.893&&0.864&0.893&0.903\tabularnewline
~~&&n&sv&&0.944&0.890&0.912&&0.811&0.815&0.800\tabularnewline
~~&&&homosc.&&0.956&0.896&0.906&&0.872&0.889&0.813\tabularnewline
~~&&u&sv&&1.057&1.151&0.869&&0.997&0.957&0.819\tabularnewline
~~&&&homosc.&&1.209&1.229&0.865&&1.233&1.149&0.870\tabularnewline
~~&lin&almon&sv&&0.959&0.892&0.964&&0.839&\textbf{0.769}&0.854\tabularnewline
~~&&&homosc.&&1.033&0.920&0.962&&0.935&0.833&0.849\tabularnewline
~~&&beta&sv&&0.934&0.855&0.924&&0.895&0.821&0.912\tabularnewline
~~&&&homosc.&&1.001&0.893&0.969&&1.005&0.927&0.985\tabularnewline
~~&&n&sv&&0.948&0.875&0.941&&0.849&0.801&0.867\tabularnewline
~~&&&homosc.&&1.018&0.904&0.939&&0.916&0.893&0.904\tabularnewline
~~&&u&sv&&0.949&0.920&1.803&&0.875&0.843&1.597\tabularnewline
~~&&&homosc.&& \shadecell 0.920&0.903&2.054&&\shadecell 1.034&0.947&1.761\tabularnewline
\bottomrule
\end{tabular}}
\caption{Inflation (GDPCTPI)}
\end{center}}
\end{table}

